A learning by confusion approach to characterize phase transitions

Recently, the learning by confusion (LBC) approach has been proposed as a machine learning tool to determine the critical temperature Tc of phase transitions without any prior knowledge of its even approximate value. However, the effectiveness of the method has been demonstrated only for continuous phase transitions, where confusion can result only from a deliberate incorrect labeling of the data and not from the coexistence of different phases. To verify whether the confusion scheme can also be used for discontinuous phase transitions, in this work, we apply the LBC method to three microscopic models, the Blume-Capel, the q-state Potts, and the Falicov-Kimball models, which undergo continuous or discontinuous phase transitions depending on model parameters. With the help of a simple model, we predict that the phase coexistence present in discontinuous phase transitions can make the neural network more confused and thus decrease its performance. However, numerical calculations performed for the models mentioned above indicate that other aspects of this kind of phase transition are more important and can render the LBC method less effective. Nevertheless, we demonstrate that in some cases the same aspects allow us to use the LBC method to identify the order of a phase transition

==> cover_bckp.tex <==
Dear Editor,

We are submitting the manuscript entitled "The Learning by Confusion approach to phase transition characterization" by Monika Richter-Laskowska, Marcin Kurpas, and Maciej M. Maśka, for publication as a regular article in Physical Review E.

The article deals with the possibility of detecting and characterizing phase transitions with the help of machine learning algorithms. In particular, we focus on the recently proposed Learning By Confusion (LBC) scheme. We tested its effectiveness in identifying continuous and discontinuous phase transitions in three qualitatively different microscopic models of interacting particles. We find that for continuous phase transitions, the method is robust and provides an accurate critical temperature for all the models. However, in the case of discontinuous transitions, its effectiveness strongly depends on the number of internal degrees of freedom of a given model. In particular, for the Falicov-Kimball model with binary degrees of freedom, the neural network learns the defects, leading to false high classification accuracy and ambiguity of the critical temperature. We show that defect recognition is related to the specific defect statistics for the Falicov-Kimball model when it undergoes a discontinuous phase transition. This aspect has not yet been discussed in the literature. 

Recent successes of machine learning algorithms in identifying phase transitions have proven their attractiveness as an alternative to standard methods, such as the Monte Carlo or exact diagonalization method. Our results indicate potential weaknesses in the use of these methods to recognize phase transitions. We believe that our manuscript contains important new results and meets the criteria for publication in Physical Review E. 

Yours sincerely,
Monika Richter-Laskowska, Marcin Kurpas, Maciej Maśka

